Avoidance of Concave Obstacles through Rotation of Nonlinear Dynamics

Controlling complex tasks in robotic systems, such as circular motion for cleaning or following curvy lines, can be dealt with using nonlinear vector fields. In this paper, we introduce a novel approach called rotational obstacle avoidance method (ROAM) for adapting the initial dynamics when the workspace is partially occluded by obstacles. ROAM presents a closed-form solution that effectively avoids star-shaped obstacles in spaces of arbitrary dimensions by rotating the initial dynamics towards the tangent space. The algorithm enables navigation within obstacle hulls and can be customized to actively move away from surfaces, while guaranteeing the presence of only a single saddle point on the boundary of each obstacle. We introduce a sequence of mappings to extend the approach for general nonlinear dynamics. Moreover, ROAM extends its capabilities to handle multi-obstacle environments and provides the ability to constrain dynamics within a safe tube. By utilizing weighted vector-tree summation, we successfully navigate around general concave obstacles represented as a tree-of-stars. Through experimental evaluation, ROAM demonstrates superior performance in terms of minimizing occurrences of local minima and maintaining similarity to the initial dynamics, outperforming existing approaches in multi-obstacle simulations. The proposed method is highly reactive, owing to its simplicity, and can be applied effectively in dynamic environments. This was demonstrated during the collision-free navigation of a 7 degree-of-freedom robot arm around dynamic obstacles

==> input/directionalmean.tex <==
\section{Preliminaries}

\subsection{Multidimensional Hyper-spheres}
A hypersphere of dimension 


\subsection{Directional Weighted Mean} \label{sec:dir_weighted_mean}
This section is a copy of \cite{huber2021avoiding}, a stereographic-inspired projection. \\
The weighted summation of vectors can result in a zero-sum, e.g., two vectors opposing each other with equal weight. If the sum of the vectors is a dynamical system for a robot motion, this can lead to local minima and undesired stopping of the agent. If the vector is used in an algorithm, the system might not be defined anymore. \\
This problem can be resolved by summing in directional space, similarly as in \cite{huber2019avoidance}. Let us define a general direction as follows:
% The modulation of the DS to avoid several obstacles as given in \cite{huber2019avoidance}, but also the continuous definition of a \textit{pseudo} normal vector requires the weighted mean of directions. With a direction $\vect v$ given as:
\begin{equation}
  \{\vect v \in \mathbb{R}^N \, :\,  \| \vect v\| = 1\} \label{eq:direction}
\end{equation}
The transformation into direction space $\mathcal{K}^{\pi}$ is given by:
\begin{equation}
\mathcal{K}^{\pi} = \{\kappa \in \mathbb{R}^{d-1} \; : \; \| \kappa \| < \pi \} \label{eq:dir_space}
\end{equation}
The direction space is with respect to a reference vector $\vect{r}^0$ which is the first column of the orthonormal transformation matrix:
\begin{equation}
  \matr R^0 =  \left[ \vect r^0  \;\; \vect e^0_1 \;\; \hdots \;\; \vect e^0_{d-1} \right] \label{eq:tranformation}
\end{equation}
This allows the transformation into a new basis:
\begin{equation}
  \hat{\vect v}^{i}= \left( \matr R^0\right)^T \vect{v}^{i} \label{eq:vector_trafo}
\end{equation}

Only the projections orthogonal to a reference vector are evaluated to evaluate the direction space. The magnitude of the transformed vector in direction space is equal to the angle between the original vector and the reference vector. The transformation of the initial vector $\vect v^i$ in the direction-space is:
\begin{equation}
  \hspace{-0.28cm}
  \kappa^i(r^0) = \vect k(\vect v^i, \vect r^0) =
  \begin{cases}
\arccos \left(\hat{ \vect{v}}^{ i}_1 \right)
\frac{\left[ \hat{\vect v}_{2}^{i} \;\; .. \;\;\; \hat{\vect v}_{d}^{i} \right]^T }{\| \left[ \hat{\vect v}_{2}^{i} \;\; .. \;\;\; \hat{\vect v}_{d}^{i} \right]^T \|}  & \text{if} \;\; \hat{ \vect{v}}^{ i}_1 \neq 1 \\
%\left[ \hat{\vect v}_{2}^{i} \;\; .. \;\;\; \hat{\vect v}_{d}^{i} \right]^T  & \text{if} \;\; \hat{ \vect{v}}^{ i}_1 =1 
\vect 0^T  & \text{if} \;\; \hat{ \vect{v}}^{ i}_1 =1 
\end{cases}
\label{eq:kappa_trafo}
\end{equation}

The mean is evaluated as a function of the weight $w^i$ of all $N^v$ vectors:
\begin{equation}
  \bar \kappa  = \sum_{i=1}^{N^v} w^i \kappa^i \label{eq:weighted_sum}
\end{equation}

The reconstruction into the original space is evaluated as follows:
\begin{equation}
  \bar{\vect v} =
  \begin{cases}
  \matr R^0
  \begin{bmatrix}
    \cos{\| \bar{ \kappa}  \|} &
    \sin{\| \bar{\kappa}} \| \frac{\bar{\kappa}}{ \| \bar{\kappa} \|}  
  \end{bmatrix}^T &   \| \bar{\kappa} \| \neq 0
  \\
  \matr R^0
  \begin{bmatrix}
    1 & 0 & .. & 0 
  \end{bmatrix}^T &  \text{if} \;  \| \bar{\kappa} \| = 0 
    \end{cases}
  \label{eq:kappa_trafo_inv}
\end{equation}


\subsubsection{Notation}
Let us refer to any vector with a bold symbol $\vect v$ (except Greek letter symbols are not printed in bold). Any direction represented in the direction space is noted with the angle-symbol $\vect v^\angle$. \\ 

Let us further refer to the process of the weighted directional mean of a set of vectors $\vect V$ with corresponding weights $W$ and null-direction $\vect{r}^0$:
\begin{equation}
\bar{\vect v} = \vect{m}_r ( \vect V, W , \vect{r}^0) = \vect{m}_r \circ ( \vect V, W , \vect{r}^0)
\end{equation}

\subsection{Mathematical Rules}
\subsubsection{Periodicity}
Since we consider direct angles, there is a periodicity of two angles, i.e., the following angle-space representations represent the same initial vector $\vect v$
\begin{equation}
    v^{\angle} + \frac{v^\angle}{\| v^\angle \|} 2 \pi n \forall n \in \mathbb{Z}\, , \; \| v^\angle \| \neq \pi k \forall k \in \mathbb{Z}
\end{equation}
the directions with magnitude $\|v^\angle\| = 2 n \pi \; \forall n \in \mathbb{Z}$ and  $\|v^\angle\| = 2 n \pi \; \forall n \in \mathbb{Z}$.

The 

\subsubsection{Relative Angle Evaluation}
Rebase to new reference base:


\subsubsection{Base Change}


\subsection{Angle Space Slerp}
Spherical linear interpolation in angle space can be done by taking the resulting vector in angles space:
\begin{equation}
\text{Slerp} = t \cdot (
\end{equation}

\subsection{Applications Beyond Dynamical Systems}


Note that there are cases where the 

Quaternion is also a 'direction' on the unit circle. Can it be represented in the angle space? What about in-between vectors?

Addition? How is it done?


\section{Loss of Information}
Many orientational descriptions lose the information of 'where it comes from.'

Including this information can lead to a 'wound-up' error, but it allows greater stability \& convergence notion.


\subesction{Desired Speed of Execution is Often Not the Real Execution}
Natural movement, i.e., speed or force of execution, differs from the desired one. The human body is intrinsically bad


==> input/literature.tex <==
\section{Literature}
%% Potential function learning (i.e. kind of create this 'valley') to ensure global convergence of the initial system.
%% () \\
Binary merging has been used to learn nonlinear motion using GMM while ensuring asymptotic convergence for trajectories contained in the continuous region $D$ containing all data points; however, the work cannot ensure that a trajectory leaves the region. Furthermore, the system requires strong conditions of the learned Gaussian distribution (such as a continuity of the data region $D$, or the correct two Gaussians being predominant in a local region) \cite{khansari2010bm}.

A popular method of learning from demonstration is SEDS \cite{khansari2012dynamical}. It ensures stability by using a quadratic Lyapunov function, however, this comes with the cost of low accuracy for non-monotonic (temporarily moving away from the attractor).
A parametrized quadratic Lyapunov function allows more complex trajectories but comes with a more complex computational cost \cite{figueroa2018physically}. However, there are still many (non-linear) trajectories that cannot be well approximated with this method.
% Limitation when trajectories are opposing in certain regions

More complex Lyapunov functions can be automatically learned to ensure the stability of the final control  \cite{khansari2014learning}. This has been further extended to additionally learn the control parameters of the motion \cite{khansari2017learning}. A weighted sum of asymmetric quadratic functions (WSAQF) is used to obtain the final Lyapunov candidate. This significantly reduces the workload of the problem, but this comes with the limitation that cannot estimate motion which is radially moving away from the attractor. Other approaches have separated the learning of global and local dynamics \cite{figueroa2022locally}, but are bound by the limits of the WSAQF, too.

Similarly, learning a contraction metric has been used to ensure the stability of a learned dynamical system \cite{sindhwani2018learning}. The parameters learned are  

The local rotation has been successfully used to learn complex and spiraling trajectory paths \cite{kronander2015incremental}. While for general paths there no limits cycles were observed, asymptotical stability towards the attractor could not be shown.

\newpage
Diffeomorphic matching of an initial linear trajectory with the learned trajectory (highly nonlinear) \cite{neumann2015learning, perrin2016fast, rana2020euclideanizing}, based on a medical image-processing algorithm \cite{joshi2000landmark}. However, the  work cannot give any guarantees on the convergence of the matching. Specifically, the diffeomorphic matching estimates spiraling trajectories with a large error.

Similarly, learning a polynomial contraction metric has been proposed to ensure the stability of a learned dynamical system \cite{ravichandar2017learning}. The approach shows good behavior on the LASA dataset, but it cannot ensure convergence to a feasible contraction metric.
% Learning partially contracting dynamical systems from demonstrations (ravichandar2017learning)

Learning contracting vector fields for stable imitation learning. Complex contraction metric to ensure a CFG (contracting vector field). Impressive figures \& application on the LASA dataset.
(\cite{sindhwani2018learning}) \\ 

%% Learning Non-Parametric Contraction Metrics of Exponentially Stable Dynamical Systems from Demonstrations (\cite{polydoros2021learning}) \\ 

Learning the orientation \& normal dynamics of a motion. This is done with contraction constraints!
(\cite{chaandar2019learning}) \\ 

% Task adaptation: Use (current) velocity to predict DS; this concept would allow to have intersecting dynamical system, where the regression is happening based on the current velocity
Continuously switching between sub-tasks just based on the current state (position and velocity) has been performed using dynamical systems 
\cite{khoramshahi2019dynamical}. While this method is not forced to follow a specific sequence, it can only choose between known sub-dynamics and not learn new ones. 

Local orientation learning allows to incrementally learn \& improve a dynamical system. A similar concept is the learning of the direction space, but on a more global level using GMM.

Linearization by considering distance (including direction) \& current velocity for the estimation of the metric. This allows a (sequential) reconstruction of the position. Allows complex \& useful diffeomorphism for Lyapunov Function / Contraction Metric Learning
(\cite{fichera2021linearization}) \\

Learning stabilizable nonlinear dynamics with contraction-based regularization. => what are the limitations (?)
\cite{singh2021learning}

% Dynamic Movement Primitives
Dynamic movement primitives introduce time-dependent parameters which ensure the convergence in finite time towards the goal\cite{ijspeert2013dynamical}. However, this leads to motion increasingly deviating from the learned motion with increasing time.

%% \subsection{Hiden Markov Model}
%% Linear parameter Varying (LPV) system, complex task sequencing using hidden Markov models (HMM) \\
%% Estimation of the dynamical system without knowing the attractor during the Expectation-Maximization-Process (E-M) \\
%% Learning subtats $s_i$ directly during the optimization step.
The division of a motion into sub-tasks which are executed an after the other using a hidden Markov model allows us to learn highly nonlinear and even crossing trajectories \cite{medina2017learning}. However, the transition to the subtask requires reaching the attractor point first, this leads to conservative position points which have to be reached. Furthermore, unexpected disturbance can lead to being in the wrong learned sub-task at the wrong position and hence to unexpected motion, even in regions with a high density of data points. 

\subsection{Funnels and Controller Design}
Motion planning using a sequence of funnels allows coping with disturbances \cite{majumdar2017funnel}. The method allows one to avoid complex environments and immediately adapt to disturbances. However, the initial optimization problem of finding the funnels cannot be guaranteed to converge. 
%% Motion planning using funnels. Stability is ensured by following these funnels. (It is not directly motion learning though \\
%% The presented present (presumably) a better trade-off between optimality and safety. 
%% () > very long paper..

\subsection{Various}
Convergence of p-dominant system (one direction sufficient to enforce convergence):
(\cite{forni2017dissipativity})

\subsection{New Work}
\cite{yao2022guiding} introduces a combined path approaching dynamics with (star-shaped) obstacle avoidance dynamics. The approach introduces a directional repulsive swirl around the obstacles, which ensures collision avoidance. However, the approach requires that the influence region of the obstacles are mutually exclusive, and has its specific distance function. Furthermore, the approach is prone to local minima in the obstacle influence region, in which case the controller switches to a non-optimal field.


\cite{lindemann2009simple} divides the space into convex sub-spaces, for which local vector fields are introduced which are ensured to flow to the desired neighboring sub-space. A graph search is then performed to find the optimal path from any subspace to the subspace containing the desired goal. This division of the space is however computationally expensive, and can not adapt to dynamic obstacles.

\cite{marcucci2021shortest}

\cite{coulombe2022generating} uses a quadratic Lyapunov function to define global stability for imitation learning. Local obstacle avoidance is ensured through the modulation of the initial dynamics.
A Neural Network is used to find a suitable Lyapunov candidate.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

